Some exact solutions in general relativity

In this thesis four separate problems in general relativity are considered, divided into two separate themes: coordinate conditions and perfect fluid spheres. Regarding coordinate conditions we present a pedagogical discussion of how the appropriate use of coordinate conditions can lead to simplifications in the form of the spacetime curvature -- such tricks are often helpful when seeking specific exact solutions of the Einstein equations. Regarding perfect fluid spheres we present several methods of transforming any given perfect fluid sphere into a possibly new perfect fluid sphere. This is done in three qualitatively distinct manners: The first set of solution generating theorems apply in Schwarzschild curvature coordinates, and are phrased in terms of the metric components: they show how to transform one static spherical perfect fluid spacetime geometry into another. A second set of solution generating theorems extends these ideas to other coordinate systems (such as isotropic, Gaussian polar, Buchdahl, Synge, and exponential coordinates), again working directly in terms of the metric components. Finally, the solution generating theorems are rephrased in terms of the TOV equation and density and pressure profiles. Most of the relevant calculations are carried out analytically, though some numerical explorations are also carried out.

==> part2_ricci.tex <==
%----------------------------------------------
%\section*{The Ricci tensor}
%----------------------------------------------
The Ricci tensor of $g_{\mu\nu}$ can then be calculated
\begin{equation}
R_{\mu\nu} =  {1\over\sqrt{-g}} \;
\left( \sqrt{-g} \;\Gamma^\sigma{}_{\mu\nu}\right)_{,\sigma}
- \left(\ln \sqrt{-g} \right)_{,\mu\nu}
- \Gamma^\rho{}_{\sigma\mu}\;\Gamma^\sigma{}_{\rho\nu}
\end{equation}
To interpret the Ricci tensor write it in $2\times2$ sub blocks
\[
R_{\mu\nu} =
\left[
\begin{array}{c|ccc}
R_{11}&R_{12}&R_{13}&R_{14}\\
\hline
R_{12}&R_{22}&R_{23}&R_{24}\\
R_{13}&R_{23}&R_{33}&R_{34}\\
R_{14}&R_{24}&R_{34}&R_{44}
\end{array}
\right]
\]
That is
\[
 R_{\mu\nu} =
\left[
\begin{array}{c|c}
R_{tt}&R_{ti}\\
\hline
R_{jt}&R_{ij}(y,z)
\end{array}
\right]
\]
Note that, since the metric is block diagonal,
\begin{equation}
g = \det[g_{\mu\nu}] = \det[f_{tt}]\;\det[h_{ij}] = -\frac{1}{N^2}\; h.
\end{equation}
Now consider
\begin{equation}
[R(g)]_{ab} =  {1\over\sqrt{-g}} \;
\left( \sqrt{-g} \;\Gamma^\sigma{}_{ab}\right)_{,\sigma}
- \left(\ln \sqrt{-g} \right)_{,ab}
- \Gamma^\rho{}_{\sigma a}\;\Gamma^\sigma{}_{\rho b}
\end{equation}
which we expand as
\begin{eqnarray}
[R(g)]_{tt} &=&
{1\over\sqrt{-f\;h}} \;
\left( \sqrt{-f\;h} \;\Gamma^t{}_{tt}\right)_{,t}
+
{1\over\sqrt{-f\;h}} \;
\left( \sqrt{-f\;h} \;\Gamma^i{}_{tt}\right)_{,i}
- \left(\ln \sqrt{-f\;h} \right)_{,tt}
\nonumber
\\
&&- \Gamma^t{}_{t t}\;\Gamma^t{}_{t t}
- \Gamma^t{}_{i t}\;\Gamma^i{}_{t t}
- \Gamma^i{}_{j t}\;\Gamma^j{}_{i t}
- \Gamma^j{}_{t t}\;\Gamma^t{}_{j t}
\nonumber
\end{eqnarray}
Then
\begin{eqnarray}
[R(g)]_{tt} &=&
{1\over\sqrt{-f}} \;
\left( \sqrt{-f} \;\Gamma^t{}_{tt}\right)_{,t} +
{1\over2} {h_{,t}\over h} \;\Gamma^t{}_{tt}
+
{1\over\sqrt{-f\;h}} \;
\left( \sqrt{-f\;h} \;\Gamma^i{}_{tt}\right)_{,i}
\nonumber
\\
&&- \left(\ln \sqrt{-f} \right)_{,tt}
- \left(\ln \sqrt{h} \right)_{,tt}
\nonumber
\\
&&- \Gamma^t{}_{t t}\;\Gamma^t{}_{t t}
- \Gamma^t{}_{i t}\;\Gamma^i{}_{t t}
- \Gamma^i{}_{j t}\;\Gamma^j{}_{i t}
- \Gamma^j{}_{t t}\;\Gamma^t{}_{j t}
\nonumber
\end{eqnarray}
which we regroup as
\begin{eqnarray}
[R(g)]_{tt} &=&
{1\over\sqrt{-f}} \;
\left( \sqrt{-f} \;\Gamma^t{}_{tt}\right)_{,t}
- \left(\ln \sqrt{-f} \right)_{,tt}
- \Gamma^t{}_{t t}\;\Gamma^t{}_{t t}
\nonumber
\\
&&+{1\over2} {h_{,t}\over h} \;\Gamma^t{}_{tt}
+{1\over\sqrt{-f\;h}} \;
\left( \sqrt{-f\;h} \;\Gamma^i{}_{tt}\right)_{,i}
- \left(\ln \sqrt{h} \right)_{,tt}
\nonumber
\\
&&- \Gamma^t{}_{i t}\;\Gamma^i{}_{t t}
- \Gamma^i{}_{j t}\;\Gamma^j{}_{i t}
- \Gamma^j{}_{t t}\;\Gamma^t{}_{j t}
\end{eqnarray}
But the first line is just $R[f]_{tt}$. The other terms can be
slightly rearranged as
\begin{eqnarray}
R_{tt} &=& [R(f)]_{tt}
- {1\over2} \left\{
\left(\ln {h} \right)_{,tt} -  {h_{,t}\over h} \;\Gamma^t{}_{tt}
\right\}
+
{1\over\sqrt{-f\;h}} \;
\left( \sqrt{-f\;h} \;\Gamma^i{}_{tt}\right)_{,i}
\nonumber
\\
&&- \Gamma^t{}_{i t}\;\Gamma^i{}_{t t}
- \Gamma^i{}_{j t}\;\Gamma^j{}_{i t}
- \Gamma^j{}_{t t}\;\Gamma^t{}_{j t}
\end{eqnarray}
Now use colons $:$ to denote 2-dimensional covariant derivatives using
the 2-metric $h$. Then
\begin{eqnarray}
[R(g)]_{tt} &=& [R(f)]_{tt}
- {1\over2} \left(\ln {h} \right)_{:tt} 
+
{1\over2} {f_{,i}\over f} \; \Gamma^i{}_{tt}
+
{1\over\sqrt{h}} \;\left( \sqrt{h} \; \Gamma^i{}_{tt}\right)_{,i}
\nonumber
\\
&&- \Gamma^t{}_{i t}\;\Gamma^i{}_{t t}
- \Gamma^i{}_{j t}\;\Gamma^j{}_{i t}
- \Gamma^j{}_{t t}\;\Gamma^t{}_{j t}
\end{eqnarray}
Now it's time to start inserting the various pieces.

Note that
\begin{equation}
{1\over\sqrt{h}} \;\left( \sqrt{h} \;\Gamma^i{}_{tt}\right)_{,i}
=-{1\over2}
{1\over\sqrt{h}} \;\left( \sqrt{h} \; h^{ij} \; \partial_j (-\frac{1}{N^2})\right)_{,i}
\end{equation}
We can write this more compactly as
\begin{equation}
{1\over\sqrt{h}} \;\left( \sqrt{h} \;\Gamma^i{}_{tt}\right)_{,i}
=
 - {1\over2}  \; \Delta_h\,(-\frac{1}{N^2}),
\end{equation}
where by $\Delta_h$ we mean the two-dimensional Laplacian in the $h$
subspace, treating the $f$ indices as though they were scalars.

Also note that
\[
\Gamma^i{}_{j t}\;\Gamma^j{}_{i t}
= {1\over 4} h^{ik} \;h_{kj,t} \;h^{jk} \;h_{ki,t}
\]
which we can re-write as
\begin{equation}
\Gamma^i{}_{j t}\;\Gamma^j{}_{i t}
= {1\over 4} h^{ik} \;h_{kj,t} \;h^{jk} \; h_{ki,t}
= {1\over 4} \tr \left[ 
{\bf h}^{-1} \; {\bf h}_{,t}  \; {\bf h}^{-1} \; {\bf h}_{,t} 
\right]
\end{equation}
and
\begin{equation}
\Gamma^t{}_{i t}\;\Gamma^i{}_{t t}
= 
-{1\over 4} N^2 \;\{(-\frac{1}{N^2})_{,i} \; h^{ij}(-\frac{1}{N^2})_{,j}\}
\end{equation}
Similarly,
\begin{equation}
\Gamma^j{}_{t t}\;\Gamma^t{}_{j t}
=
-{1\over 4} N^2 \;\{(-\frac{1}{N^2})_{,i} \; h^{ji}(-\frac{1}{N^2})_{,j}\}
\end{equation}
Finally
\begin{equation}
{f_{,i}\over f} \; \Gamma^i{}_{tt}=
-{1\over2}{f_{,i}\over f}\; h^{ij}\{(-\frac{1}{N^2})_{,j}\} 
\end{equation}
Now pull all these pieces together.
\begin{eqnarray}
[R(g)]_{tt} &=& [R(f)]_{tt}
- {1\over 2} \left(\ln {h} \right)_{:tt}    - {1\over2}  \; \Delta_h\,(-\frac{1}{N^2})
-{1\over 4} \tr \left[ 
{\bf h}^{-1} \; {\bf h}_{,t}  \; {\bf h}^{-1} \; {\bf h}_{,t} 
\right]
\nonumber
\\
&&-{1\over 4}  {f_{,i}\over f}\; h^{ij}\{(-\frac{1}{N^2})_{,j}\}
+{1\over 4} N^2 \;\{(-\frac{1}{N^2})_{,i} \; h^{ij}(-\frac{1}{N^2})_{,j}\}
\nonumber
\\
&&+{1\over 4} N^2 \;\{(-\frac{1}{N^2})_{,i} \; h^{ji}(-\frac{1}{N^2})_{,j}\}
\end{eqnarray}
There are still simplifications.  For instance
\begin{equation}
\left(\ln {h} \right)_{:tt} = \left( {h_{:t}\over h}\right)_{:t} 
= {h_{:tt}\over h} - {h_{:t} \over h} \; {h_{:t}\over h}
\end{equation}
gets rid of the logarithm. Then
\begin{eqnarray}
[R(g)]_{tt} &=& [R(f)]_{tt}
- {1\over2} {h_{:tt}\over h}
+{1\over2} {h_{:t} \over h} \; {h_{:t}\over h}
- {1\over2} \; \Delta_h\,(-\frac{1}{N^2})
\\
&& -{1\over 4} \tr \left[ 
{\bf h}^{-1} \; {\bf h}_{,t}  \; {\bf h}^{-1} \; {\bf h}_{,t} \right] 
-{1\over 4}{f_{,i}\over f}\; h^{ij}\{(-\frac{1}{N^2})_{,j}\}
\nonumber
\\
&& +{1\over 4} N^2 \;\{(-\frac{1}{N^2})_{,i} \; h^{ij}(-\frac{1}{N^2})_{,j}\}
+{1\over 4} N^2 \;\{(-\frac{1}{N^2})_{,i} \; h^{ji}(-\frac{1}{N^2})_{,j}\}
\nonumber
\end{eqnarray}
For $[R(g)]_{ij}$ is can simply write:
\begin{eqnarray}
[R(g)]_{ij} &=& [R(h)]_{ij} 
- {1\over2} {f_{|ij}\over f} 
+{1\over2}  {f_{|i} \over f} \; {f_{|j}\over f}
- {1\over2} \; \Delta_f\, h_{ij}
-{1\over 4} \tr \left[
{\bf f}^{-1} \; {\bf f}_{,i}  \; {\bf f}^{-1} \; {\bf f}_{,j} 
\right]
\\
&&-{1\over4}  {h_{,t}\over h}\; (-N^2) h_{ij,t}
-{1\over 4} h^{ki} \; (h_{ki,t} \; N^2 \; h_{ij,t})
-{1\over 4} h^{ik} \; (h_{ki,t} \; N^2 \; h_{ij,t})
\nonumber
\end{eqnarray}
But then
\begin{eqnarray}
f^{tt} \; [R(g)]_{tt} &=& f^{tt} \; [R(f)]_{tt} 
- {1\over2} {\Delta_f\,h\over h} 
+{1\over2}  {h_{:t} \over h} \; {h^{:t}\over h}
- {1\over2}   f^{tt} \Delta_h\,(-\frac{1}{N^2})
\nonumber
\\
&&- {1\over 4}  f^{tt} \; \tr \left[ 
{\bf h}^{-1} \; {\bf h}_{,t}  \; {\bf h}^{-1} \; {\bf h}_{,t} \right]
-{1\over4} {f_{|i} \over f}\;  {f^{|i}\over f}
\nonumber
\\
&& - {1\over 4}  h^{ij} \;
\tr \left[ 
{\bf f}^{-1} \; {\bf f}_{,i}  \; {\bf f}^{-1} \; {\bf f}_{,j}
\right]
- {1\over 4}  h^{ji} \;
\tr \left[ 
{\bf f}^{-1} \; {\bf f}_{,i}  \; {\bf f}^{-1} \; {\bf f}_{,j} 
\right]
\end{eqnarray}
with a similar formula holding for $h^{ij}\;[R(g)]_{ij}$:
\begin{eqnarray}
h^{ij} \; [R(g)]_{ij} &=& h^{ij} \; [R(h)]_{ij} 
- {1\over2} {\Delta_h\,f\over f} 
+{1\over2}  {f_{|i} \over f} \; {f^{|i}\over f}
 - {1\over2}   h^{ij} \; \Delta_f\, h_{ij}
\nonumber
\\
&& - {1\over 4}  h^{ij} \; \tr \left[
{\bf f}^{-1} \; {\bf f}_{,i}  \; {\bf f}^{-1} \; {\bf f}_{,j} 
\right]
-{1\over4} {h_{|t} \over h}\;  {h^{|t}\over h}
\nonumber
\\
&& - {1\over 4}  N^2\;
\tr \left[
{\bf h}^{-1} \; {\bf h}_{,t}  \; {\bf h}^{-1} \; {\bf h}_{,t}
\right]
- {1\over 4} \;h^{ij} \;h^{ik} \; (h_{ki,t} \; N^2 \; h_{ij,t})
\end{eqnarray}
Then in the Ricci scalar there are a lot of partial cancellations
\begin{eqnarray}
R(g) &=&  f^{tt} \; [R(g)]_{tt}  + h^{ij}\;[R(g)]_{ij} 
\nonumber
\\
&=& R(h) + R(f) - {1\over2} {\Delta_f\,h\over h} - {1\over2} {\Delta_h\,f\over f} 
+{1\over4}  {h_{:t} \over h} \; {h^{:h}\over h}
+{1\over4}  {f_{|i} \over f} \; {f^{|i}\over f}
\nonumber
\\
&&- {1\over2}   f^{tt} \; \Delta_h\, (-\frac{1}{N^2})
- {1\over2}  h^{ij} \; \Delta_f\, h_{ij}
 -{1\over 2}  h^{ij} \; \tr \left[ 
{\bf f}^{-1} \; {\bf f}_{,i}  \; {\bf f}^{-1} \; {\bf f}_{,j} 
\right]
\nonumber
\\
&& - {1\over 4}  h^{ji} \;
\tr \left[
{\bf f}^{-1} \; {\bf f}_{,i}  \; {\bf f}^{-1} \; {\bf f}_{,j} 
\right]
-{1\over 4} h^{ij} h^{ik} \; (h_{ki,t} \; N^2 \; h_{ij,t})
\end{eqnarray}
%---------------------------------------------------

==> references.tex <==
%----------------------------------------------------------------------
\begin{thebibliography}{99}
%----------------------------------------------------------------------
% Background

\bibitem{Delgaty}
M.~S.~R.~Delgaty and K.~Lake,
``Physical acceptability of isolated, static, spherically symmetric,  perfect
fluid solutions of Einstein's equations,''
Comput.\ Phys.\ Commun.\  {\bf 115} (1998) 395
[arXiv:gr-qc/9809013].
%%CITATION = GR-QC 9809013;%%

\bibitem{Skea}
M.~R.~Finch and J.~E.~F.~Skea,
``A review of the relativistic static fluid sphere'',
1998, unpublished.\\*
{\sf http://www.dft.if.uerj.br/usuarios/JimSkea/papers/pfrev.ps}



\bibitem{exact}
H. Stephani, D. Kramer, M. MacCallum, C. Hoenselaers, and E. Herlt,
\emph{Exact solutions of Einstein's field equations},
  (Cambridge University Press, 2003).

\bibitem{Martin0}
D.~Martin and M.~Visser,
``Bounds on the interior geometry and pressure profile of static fluid
spheres,''
Class.\ Quant.\ Grav.\  {\bf 20} (2003) 3699
[arXiv:gr-qc/0306038].
%%CITATION = GR-QC 0306038;%%


% History


\bibitem{Buchdahl} 
H.~A.~Buchdahl,
``General Relativistic fluid spheres'',
Phys.~Rev.~{\bf 116} (1959) 1027--1034;
\\
``General Relativistic fluid spheres II: 
general inequalities for regular spheres'',
Ap. J. {\bf 146} (1966) 275--281.


\bibitem{Bondi}
H.~Bondi,
``Spherically Symmetrical Models In General Relativity'',
Mon.~Not.~Roy.~Astron.~Soc.~ {\bf 107} (1947) 410.
%%CITATION = MNRAA,107,410;%%
\\
``Massive spheres in general relativity'',
Mon.~Not.~Roy.~Astron.~Soc.  {\bf 282} (1964) 303--317.

\bibitem{Wyman}
M. Wyman, 
``Radially symmetric distributions of matter'',
Phys. Rev. {\bf 75} (1949) 1930. 

\bibitem{Hojman-et-al}
S.~Berger, R.~Hojman and J.~Santamarina,
``General Exact Solutions Of Einstein Equations For 
Static Perfect Fluids With Spherical Symmetry,''
J.\ Math.\ Phys.\  {\bf 28} (1987) 2949.
%%CITATION = JMAPA,28,2949;%%


% Recent

\bibitem{Rahman}
S.~Rahman and M.~Visser,
``Spacetime geometry of static fluid spheres,''
Class.\ Quant.\ Grav.\  {\bf 19} (2002) 935
[arXiv:gr-qc/0103065].
%%CITATION = GR-QC 0103065;%%


\bibitem{Lake}
K.~Lake,
``All static spherically symmetric perfect fluid solutions of Einstein's
Equations,''
Phys.\ Rev.\ D {\bf 67} (2003) 104015
[arXiv:gr-qc/0209104].
%%CITATION = GR-QC 0209104;%%


\bibitem{Martin}
D.~Martin and M.~Visser,
``Algorithmic construction of static perfect fluid spheres,''
Phys.\ Rev.\ D {\bf 69} (2004) 104028
[arXiv:gr-qc/0306109].
%%CITATION = GR-QC 0306109;%%

%----------------------------------------------------------------------
\end{thebibliography}
%-----------------------------------------------------------------------

%------------------------------------------------
%\end{document}
%-----------------------------------------------
% EOF algorithm.tex
%-----------------------------------------------


